Cluster-Guided Semi-Supervised Domain Adaptation for Imbalanced Medical Image Classification

Semi-supervised domain adaptation is a technique to build a classifier for a target domain by modifying a classifier in another (source) domain using many unlabeled samples and a small number of labeled samples from the target domain. In this paper, we develop a semi-supervised domain adaptation method, which has robustness to class-imbalanced situations, which are common in medical image classification tasks. For robustness, we propose a weakly-supervised clustering pipeline to obtain high-purity clusters and utilize the clusters in representation learning for domain adaptation. The proposed method showed state-of-the-art performance in the experiment using severely class-imbalanced pathological image patches.

==> related_work.tex <==
\section{Related work}
\label{sec:review}
\noindent{\bf Unsupervised domain adaptation}:\ 
Many unsupervised domain adaptation~(UDA) methods have been reported~\cite{Gretton2009mit,Long2015icml,Yaroslav2015icml,tzeng2017cvpr,tang2020aaai,wang2021pr}. 
A famous approach for UDA is to use an adversarial loss~\cite{Yaroslav2015icml,tzeng2017cvpr,tang2020aaai,Shuhan2020,wang2021pr}. This approach introduces a domain classifier that classifies whether the input data is sampled from the source or target domain and aligns the distribution of the two domains by training the feature extractor to obtain feature representations that the domain classifier misclassifies. For example, Ganin~\textit{et al.}~\cite{Yaroslav2015icml} proposed the gradient reversal algorithm to obtain feature representations that are misclassified by a domain classifier. In recent years, Tan~\textit{et al.} have proposed COAL, which considers class imbalance of a dataset~\cite{Shuhan2020}. They reviewed the data sampling method to deal with class imbalance, and COAL uses class-balanced mini-batch sampling.
\par
The existing method is difficult to train in fundamentally difficult tasks such as medical image diagnosis using pathological images because it assumes that each class of the target domain can be roughly separated in the feature space of the model trained only with the source domain.
\par
\noindent{\bf Semi-supervised domain adaptation}:\ 
Several recent studies have reported semi-supervised domain adaptation~(SSDA), which combines semi-supervised learning and domain adaption~\cite{saito2019semi,Pin2020ijcai,He2020cvprws,li2021ECACL}. Many existing SSDA methods are based on adversarial training. For example, Saito~\textit{et al.} proposed MME~\cite{saito2019semi}, which maximizes the entropy of the class probability of the unlabeled target samples predicted from the model and minimizes the entropy of the feature extractor to obtain a feature representation that is easy to classify. Li~\textit{et al.} proposed ECACL, which uses Triplet loss to align samples of each class in source and target domains~\cite{li2021ECACL}. In our work, a pair of three samples is used for representation learning. Unlike ECACL, which uses it to align the labeled source and target samples as supervised learning, the proposed method is used to align clusters of target samples to the source domain.
\par
Several studies have been reported on SSDA considering clusters of samples~\cite{li2021cross,singh2021clda}. Singh proposed CLDA, which aligns the distribution of both domains using the centroid of each class in each domain~\cite{singh2021clda}. In addition, Li~\textit{et al.} proposed CDAC, which uses the similarity between unlabeled target samples~\cite{li2021cross}. Although these methods have improved classification performance, they do not consider class imbalance that class label distribution follows a long-tailed distribution such as the Pareto distribution~\cite{William2001}. To the best of our knowledge, this work is the first report on SSDA problems with class imbalance.
\par
\noindent{\bf Domain adaptation for medical diagnosis}:\ 
The UDA framework for medical data tasks has been reported by many studies~\cite{Jian2018miccai,perone2019ni,Yifan2020ti,jinpeng2020tcds,Hao2021tbme}. Zhang~\textit{et al.} proposed a UDA method for medical image diagnosis~\cite{Yifan2020ti}. Their method assumed that the data may have noise labels and could eliminate hard-to-adaptation samples. Moreover, Li~\textit{et al.} proposed domain adaptation method for EEG signals~\cite{jinpeng2020tcds}. Their method uses adversarial training to align the distributions of the source and the target domain in the early layers and align the distribution of each class in the last layer.
\par
The UDA and SSDA methods described above work well on a class-balanced dataset, but in many cases, they do not work on a class-imbalanced dataset. For example, when using adversarial loss, it would be easy to have a situation where unlabeled target samples with a minority class may align the distribution of the source sample with a majority class. The proposed method deals with class imbalance situations by considering the class proportion of the labeled target samples.
% \begin{figure*}[t]
% \center
% \includegraphics[width=\textwidth]{./figs/steps-small.pdf}
% \caption{Outline of the proposed weakly-supervised clustering. The weakly-supervised clustering consists of three steps. The first step is k-means clustering is performed for labeled and unlabeled target samples. The second step is cluster refinement by soft-constrained clustering, which re-clustering a cluster containing different class samples. The third step is cluster refinement by proportion-based splitting, which splits a cluster into smaller clusters according to class proportions.
% } 
% \label{fig:clustering-outline}
% \end{figure*}
